Real-Time Model Predictive Control for Energy Management in Autonomous Underwater Vehicle

Improving endurance is crucial for extending the spatial and temporal operation range of autonomous underwater vehicles (AUVs). Considering the hardware constraints and the performance requirements, an intelligent energy management system is required to extend the operation range of AUVs. This paper presents a novel model predictive control (MPC) framework for energy-optimal point-to-point motion control of an AUV. In this scheme, the energy management problem of an AUV is reformulated as a surge motion optimization problem in two stages. First, a system-level energy minimization problem is solved by managing the trade-off between the energies required for overcoming the positive buoyancy and surge drag force in static optimization. Next, an MPC with a special cost function formulation is proposed to deal with transients and system dynamics. A switching logic for handling the transition between the static and dynamic stages is incorporated to reduce the computational efforts. Simulation results show that the proposed method is able to achieve near-optimal energy consumption with considerable lower computational complexity.

==> Reference <==
@inproceedings{Iscar:2018aa,
	Author = {Eduardo Iscar and Corina Barbalata and Nicholas Goumas and M. Johnson-Roberson},
	Booktitle = {{IEEE/MTS Oceans}},
	Date-Added = {2018-08-17 04:38:19 +0000},
	Date-Modified = {2018-08-17 04:39:13 +0000},
	Keywords = {conf},
	Title = {Towards low cost, deep water AUV optical mapping},
	Year = {2018}}

@article{eriksen2001seaglider,
  title={Seaglider: A long-range autonomous underwater vehicle for oceanographic research},
  author={Eriksen, Charles C and Osse, T James and Light, Russell D and Wen, Timothy and Lehman, Thomas W and Sabin, Peter L and Ballard, John W and Chiodi, Andrew M},
  journal={IEEE Journal of oceanic Engineering},
  volume={26},
  number={4},
  pages={424--436},
  year={2001},
  publisher={IEEE}
}

@article{webb2001slocum,
  title={SLOCUM: An underwater glider propelled by environmental energy},
  author={Webb, Douglas C and Simonetti, Paul J and Jones, Clayton P},
  journal={IEEE Journal of oceanic engineering},
  volume={26},
  number={4},
  pages={447--452},
  year={2001},
  publisher={IEEE}
}

@article{santhakumar2013power,
  title={Power efficient dynamic station keeping control of a flat-fish type autonomous underwater vehicle through design modifications of thruster configuration},
  author={Santhakumar, Mohan and Asokan, Thondiyath},
  journal={Ocean Engineering},
  volume={58},
  pages={11--21},
  year={2013},
  publisher={Elsevier}
}


@article{hasvold2004clipper,
  title={CLIPPER: a long-range, autonomous underwater vehicle using magnesium fuel and oxygen from the sea},
  author={Hasvold, {\O}istein and Lian, Torleif and Haakaas, Erik and St{\o}rkersen, Nils and Perelman, Olivier and Cordier, Stephane},
  journal={Journal of power sources},
  volume={136},
  number={2},
  pages={232--239},
  year={2004},
  publisher={Elsevier}
}

@incollection{subramani2015stochastic,
  title={A stochastic optimization method for energy-based path planning},
  author={Subramani, Deepak N and Lolla, Tapovan and Haley, Patrick J and Lermusiaux, Pierre FJ},
  booktitle={Dynamic Data-Driven Environmental Systems Science},
  pages={347--358},
  year={2015},
  publisher={Springer}
}

@inproceedings{garau2005path,
  title={Path planning of autonomous underwater vehicles in current fields with complex spatial variability: an A* approach},
  author={Garau, Bartolome and Alvarez, Alberto and Oliver, Gabriel},
  booktitle={Robotics and Automation, 2005. ICRA 2005. Proceedings of the 2005 IEEE International Conference on},
  pages={194--198},
  year={2005},
  organization={IEEE}
}

@article{alvarez2004evolutionary,
  title={Evolutionary path planning for autonomous underwater vehicles in a variable ocean},
  author={Alvarez, Alberto and Caiti, Andrea and Onken, Reiner},
  journal={IEEE Journal of Oceanic Engineering},
  volume={29},
  number={2},
  pages={418--429},
  year={2004},
  publisher={IEEE}
}

@inproceedings{witt2008go,
  title={Go with the flow: Optimal AUV path planning in coastal environments},
  author={Witt, Jonas and Dunbabin, Matthew},
  booktitle={Australian Conference on Robotics and Automation},
  volume={2008},
  number={2},
  year={2008}
}

@article{subramani2017energy,
  title={Energy-optimal path planning in the coastal ocean},
  author={Subramani, Deepak N and Haley, Patrick J and Lermusiaux, Pierre FJ},
  journal={Journal of Geophysical Research: Oceans},
  volume={122},
  number={5},
  pages={3981--4003},
  year={2017},
  publisher={Wiley Online Library}
}

@article{sarkar2016modelling,
  title={Modelling and simulation of a robust energy efficient AUV controller},
  author={Sarkar, M and Nandy, S and Vadali, SRK and Roy, Spandan and Shome, SN},
  journal={Mathematics and Computers in Simulation},
  volume={121},
  pages={34--47},
  year={2016},
  publisher={Elsevier}
}

@article{geranmehr2015nonlinear,
  title={Nonlinear suboptimal control of fully coupled non-affine six-DOF autonomous underwater vehicle using the state-dependent Riccati equation},
  author={Geranmehr, Behdad and Nekoo, Saeed Rafee},
  journal={Ocean Engineering},
  volume={96},
  pages={248--257},
  year={2015},
  publisher={Elsevier}
}

@article{mayne2000constrained,
  title={Constrained model predictive control: Stability and optimality},
  author={Mayne, David Q and Rawlings, James B and Rao, Christopher V and Scokaert, Pierre OM},
  journal={Automatica},
  volume={36},
  number={6},
  pages={789--814},
  year={2000},
  publisher={Elsevier}
}

@article{garcia1989model,
  title={Model predictive control: theory and practice—a survey},
  author={Garcia, Carlos E and Prett, David M and Morari, Manfred},
  journal={Automatica},
  volume={25},
  number={3},
  pages={335--348},
  year={1989},
  publisher={Elsevier}
}

@book{wadoo2017autonomous,
  title={Autonomous underwater vehicles: modeling, control design and simulation},
  author={Wadoo, Sabiha and Kachroo, Pushkin},
  year={2017},
  publisher={CRC Press}
}

@article{yuh1990modeling,
  title={Modeling and control of underwater robotic vehicles},
  author={Yuh, Junku},
  journal={IEEE Transactions on Systems, man, and Cybernetics},
  volume={20},
  number={6},
  pages={1475--1483},
  year={1990},
  publisher={IEEE}
}

@article{reyhanoglu1999dynamics,
  title={Dynamics and control of a class of underactuated mechanical systems},
  author={Reyhanoglu, Mahmut and van der Schaft, Arjan and McClamroch, N Harris and Kolmanovsky, Ilya},
  journal={IEEE Transactions on Automatic Control},
  volume={44},
  number={9},
  pages={1663--1671},
  year={1999},
  publisher={IEEE}
}

@Misc{timmurphy.org,  
howpublished = {\url{http://www.starlino.com/power2thrust.html}},  
note = {Accessed February 12, 2018},  
title = {How much power is needed to hovering},  
author = {Sergiu Baluta}  
}  

@article{jagtap2016control,
  title={Control of autonomous underwater vehicle using reduced order model predictive control in three dimensional space},
  author={Jagtap, Pushpak and Raut, Pranoti and Kumar, Pawan and Gupta, Ankit and Singh, NM and Kazi, Faruk},
  journal={IFAC-PapersOnLine},
  volume={49},
  number={1},
  pages={772--777},
  year={2016},
  publisher={Elsevier}
}

@article{von1992direct,
  title={Direct and indirect methods for trajectory optimization},
  author={Von Stryk, Oskar and Bulirsch, Roland},
  journal={Annals of operations research},
  volume={37},
  number={1},
  pages={357--373},
  year={1992},
  publisher={Springer}
}

@article{goheen1990multivariable,
  title={Multivariable self-tuning autopilots for autonomous and remotely operated underwater vehicles},
  author={Goheen, Kevin R and Jefferys, E Richard},
  journal={IEEE Journal of Oceanic Engineering},
  volume={15},
  number={3},
  pages={144--151},
  year={1990},
  publisher={IEEE}
}

@article{repoulias2007planar,
  title={Planar trajectory planning and tracking control design for underactuated AUVs},
  author={Repoulias, Filoktimon and Papadopoulos, Evangelos},
  journal={Ocean Engineering},
  volume={34},
  number={11-12},
  pages={1650--1667},
  year={2007},
  publisher={Elsevier}
}

@article{chyba2009increasing,
  title={Increasing underwater vehicle autonomy by reducing energy consumption},
  author={Chyba, M and Haberkorn, T and Singh, SB and Smith, RN and Choi, SK},
  journal={Ocean Engineering},
  volume={36},
  number={1},
  pages={62--73},
  year={2009},
  publisher={Elsevier}
}

@inproceedings{bellingham1990keeping,
  title={Keeping layered control simple (autonomous underwater vehicles)},
  author={Bellingham, James G and Consi, Thomas R and Beaton, Robert M and Hall, William},
  booktitle={Autonomous Underwater Vehicle Technology, 1990. AUV'90., Proceedings of the (1990) Symposium on},
  pages={3--8},
  year={1990},
  organization={IEEE}
}

@article{shen2016diving,
  title={Diving control of autonomous underwater vehicle based on improved active disturbance rejection control approach},
  author={Shen, Yuxuan and Shao, Keyong and Ren, Weijian and Liu, Yurong},
  journal={Neurocomputing},
  volume={173},
  pages={1377--1385},
  year={2016},
  publisher={Elsevier}
}

@article{musardo2005ecms,
  title={A-ECMS: An adaptive algorithm for hybrid electric vehicle energy management},
  author={Musardo, Cristian and Rizzoni, Giorgio and Guezennec, Yann and Staccia, Benedetto},
  journal={European Journal of Control},
  volume={11},
  number={4-5},
  pages={509--524},
  year={2005},
  publisher={Elsevier}
}

@inproceedings{luo2013improved,
  title={An improved parameterized approach for real time optimal motion planning of AUV moving in dynamic environment},
  author={Luo, Wenhao and Peng, Jun and Wang, Jing},
  booktitle={Robotics, Automation and Mechatronics (RAM), 2013 6th IEEE Conference on},
  pages={103--108},
  year={2013},
  organization={IEEE}
}

@article{wojsznis2003practical,
  title={Practical approach to tuning MPC},
  author={Wojsznis, Willy and Gudaz, John and Blevins, Terry and Mehta, Ashish},
  journal={ISA transactions},
  volume={42},
  number={1},
  pages={149--162},
  year={2003},
  publisher={Elsevier}
}

@article{cagienard2007move,
  title={Move blocking strategies in receding horizon control},
  author={Cagienard, Raphael and Grieder, Pascal and Kerrigan, Eric C and Morari, Manfred},
  journal={Journal of Process Control},
  volume={17},
  number={6},
  pages={563--570},
  year={2007},
  publisher={Elsevier}
}

@book{bellman2013dynamic,
  title={Dynamic programming},
  author={Bellman, Richard},
  year={2013},
  publisher={Courier Corporation}
}

@inproceedings{lee2011model,
  title={Model predictive control and dynamic programming},
  author={Lee, Jay H},
  booktitle={Control, Automation and Systems (ICCAS), 2011 11th International Conference on},
  pages={1807--1809},
  year={2011},
  organization={IEEE}
}

@article{rawlings2009model,
  title={Model predictive control: Theory and design},
  author={Rawlings, James B and Mayne, David Q},
  year={2009},
  publisher={Nob Hill Pub. Madison, Wisconsin}
}

@phdthesis{prestero2001verification,
  title={Verification of a six-degree of freedom simulation model for the REMUS autonomous underwater vehicle},
  author={Prestero, Timothy Timothy Jason},
  year={2001},
  school={Massachusetts institute of technology}
}
